Identifying Stereotypes in the Online Perception of Physical Attractiveness

Stereotyping can be viewed as oversimplified ideas about social groups. They can be positive, neutral or negative. The main goal of this paper is to identify stereotypes for female physical attractiveness in images available in the Web. We look at the search engines as possible sources of stereotypes. We conducted experiments on Google and Bing by querying the search engines for beautiful and ugly women. We then collect images and extract information of faces. We propose a methodology and apply it to analyze photos gathered from search engines to understand how race and age manifest in the observed stereotypes and how they vary according to countries and regions. Our findings demonstrate the existence of stereotypes for female physical attractiveness, in particular negative stereotypes about black women and positive stereotypes about white women in terms of beauty. We also found negative stereotypes associated with older women in terms of physical attractiveness. Finally, we have identified patterns of stereotypes that are common to groups of countries.

==> datasets.tex <==
\section{Datasets}
\label{sec:data}

In this section we present a brief characterization of the datasets collected for this work using the methodology described in the section~\ref{sec:methodData}. As mentioned, we picked the top 50 photos for each query but we consider as valid only images for which Face++ was able to detect a unique face (see appendix~\ref{app1}). The characterization and analysis will be performed for all countries which the queries have over 20 valid photos.

For first part of the characterization our aim is to show the proportion of the races by country.  The Figure~\ref{propGoogle} shows this proportion for the 42 countries for which we performed searches on Google and in the Figure~\ref{propBing} the 17 countries for Bing. The first observation we can do from charts is that clearly the proportion of black women in search 'ugly women' is greater, in general, for the two search engines. We have also calculated the mean and standard deviation of each race for both queries and search engines. From the results of Table~\ref{tabMeanStDv} we observed that this behavior is the same for Asian women. 

\begin{figure}[!h]
  \begin{subfigure}[t]{0.4\textwidth}
          \centering
          \includegraphics[scale=0.35]{fig/propBeautyGoogle.png}
          \label{propBeautyGoogle}
  \end{subfigure}
	\hspace{3em}
  \begin{subfigure}[t]{0.4\textwidth}
          \centering
          \includegraphics[scale=0.35]{fig/propUglyGoogle.png}   
          \label{propUglyGoogle}
  \end{subfigure}
  \caption{Race Proportions for Google.} 
  \label{propGoogle}
\end{figure} 

\begin{figure}[!h]
  \begin{subfigure}[t]{0.4\textwidth}
          \centering
          \includegraphics[scale=0.35]{fig/propBeautyBing.png}
      %\caption{}   
          \label{propBeautyBing}
  \end{subfigure}
	\hspace{3em}
  \begin{subfigure}[t]{0.4\textwidth}
          \centering
          \includegraphics[scale=0.35]{fig/propUglyBing.png}
      %\caption{}   
          \label{propUglyBing}
  \end{subfigure}
  \caption{Race Proportions for Bing.} 
  \label{propBing}
\end{figure}

\begin{table}[!h]
\centering
\begin{scriptsize}
\caption{Mean and Standard Deviation of Proportions}
\label{tabMeanStDv}
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{12}{c}{\textbf{Google}}                                  \\ \hline
\multicolumn{6}{c|}{\textit{\textbf{beautiful woman}}}                                                                                                                     & \multicolumn{6}{c}{\textit{\textbf{ugly woman}}}                                                                                                      \\ \hline
\multicolumn{2}{c|}{\textit{Asian}}                     & \multicolumn{2}{c|}{\textit{Black}}                    & \multicolumn{2}{c|}{\textit{White}}                     & \multicolumn{2}{c|}{\textit{Asian}}                     & \multicolumn{2}{c|}{\textit{Black}}                    & \multicolumn{2}{c}{\textit{White}} \\ \hline
\multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv}  & \multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv} & \multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv}  & \multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv}  & \multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv} & \multicolumn{1}{c|}{mean}   & stdv \\ \hline
\multicolumn{1}{c|}{13.77} & \multicolumn{1}{c|}{15.65} & \multicolumn{1}{c|}{2.37}  & \multicolumn{1}{c|}{5.99} & \multicolumn{1}{c|}{83.86} & \multicolumn{1}{c|}{16.96} & \multicolumn{1}{c|}{15.36} & \multicolumn{1}{c|}{11.48} & \multicolumn{1}{c|}{19.20} & \multicolumn{1}{c|}{9.23} & \multicolumn{1}{c|}{65.44}  & 9.48 \\
                           &                            &                            &                           &                            &                            &                            &                            &                            &                           &                             &      \\ \hline
\multicolumn{12}{c}{\textbf{Bing}}                                                                                                                                                                                                                                                                                                 \\ \hline
\multicolumn{6}{c|}{\textit{\textbf{beautiful woman}}}                                                                                                                     & \multicolumn{6}{c}{\textit{\textbf{ugly woman}}}                                                                                                      \\ \hline
\multicolumn{2}{c|}{\textit{Asian}}                     & \multicolumn{2}{c|}{\textit{Black}}                    & \multicolumn{2}{c|}{\textit{White}}                     & \multicolumn{2}{c|}{\textit{Asian}}                     & \multicolumn{2}{c|}{\textit{Black}}                    & \multicolumn{2}{c}{\textit{White}} \\ \hline
\multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv}  & \multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv} & \multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv}  & \multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv}  & \multicolumn{1}{c|}{mean}  & \multicolumn{1}{c|}{stdv} & \multicolumn{1}{c|}{mean}   & stdv \\ \hline
\multicolumn{1}{c|}{12.96} & \multicolumn{1}{c|}{11.82} & \multicolumn{1}{c|}{03.09} & \multicolumn{1}{c|}{2.59} & \multicolumn{1}{c|}{83.94} & \multicolumn{1}{c|}{11.78} & \multicolumn{1}{c|}{15.35} & \multicolumn{1}{c|}{5.19}  & \multicolumn{1}{c|}{15.63} & \multicolumn{1}{c|}{8.54} & \multicolumn{1}{c|}{69.02}  & 5.19
\end{tabular}
\end{scriptsize}
\end{table}

The second part of the characterization shows the difference between the age distribution of women in photos by query and search engine through boxplots (Figure~\ref{distGoogle} and ~\ref{distBing}). In the x-axis we have the analyzed countries and the y-axis represents ages. Noting the median and upper quartile we noticed that beautiful women tend to be younger than the ugly women.

\begin{figure}[!h]
  \begin{subfigure}[b]{0.55\textwidth}
          \centering
          \includegraphics[scale=0.25]{fig/distBeautyGoogle.png}
      %\caption{}   
          \label{distBeautyGoogle}
  \end{subfigure}
  \newline
  \begin{subfigure}[b]{0.55\textwidth}
          \centering
          \includegraphics[scale=0.25]{fig/distUglyGoogle}
      %\caption{}   
          \label{distUglyGoogle}
  \end{subfigure}
  \caption{Age distribution for Google.} 
  \label{distGoogle}
\end{figure}

\begin{figure}[!h]
  \begin{subfigure}[b]{0.55\textwidth}
          \centering
          \includegraphics[scale=0.3]{fig/distBeautyBing.png}
      %\caption{}   
          \label{distBeautyBing}
  \end{subfigure}
  \newline
  \begin{subfigure}[b]{0.55\textwidth}
          \centering
          \includegraphics[scale=0.3]{fig/distUglyBing}
      %\caption{}   
          \label{distUglyBing}
  \end{subfigure}
  \caption{Age distribution for Bing.} 
  \label{distBing}
\end{figure}


==> method.tex <==
\section{Methodology}
\label{sec:method}

In this section we describe the methodology used for characterizing stereotypes. We use a database of photos and information extracted from these photos, in particular features of the people portrayed. The first step of the methodology involves the data collection process: what and how to collect the data. Then we extract information about the collected photos, using computer vision algorithms to identify race, age and gender of the people in each picture. The second part of the research refers to the use of  the collected information to identify stereotypes.

\subsection{Data Gathering}
\label{sec:methodData}

This work is based on the analysis of photos, thus the data gathering was carried through two search engines APIs for images: Google and Bing. In order to extract features from the photos, we used Face++\footnote{http://www.faceplusplus.com/}. 

The data gathering process is depicted in Figure~\ref{frame} and is summarized next:

\begin{small}
\begin{enumerate}
\item Build search query\\
For the specific context, beauty, select the relevant search queries and translate the query into the target languages.
\item Gathering\\Using the search engines APIs, perform the searches with the predefined queries. Filter photos that contain the face of just one person.
\item Extract attributes of photos\\Using face detection tools estimate race, age and gender.
\end{enumerate}
\end{small}

\begin{figure}[!h]
        \centering
        \includegraphics[scale=0.32]{fig/frame.png}
   	\caption{Data Gathering Framework.}   
		\label{frame}
\end{figure}

For the beauty context we collected the top 50 photos of the results of the following queries (in different languages): beautiful woman and ugly woman. Beauty is a property, or set of properties, that makes someone capable of producing a certain sort of pleasurable experience in any suitable perceiver \cite{TCDP1999}. It is known that what is defined as beautiful or ugly might change from person to person, then we chose these two antonyms adjectives that are commonly used to describe the quality of beauty of people.

Bing's API offers the option of 22 countries to perform the searches, we collected data for all these countries. For Google we collected data for the same 22 countries and added more countries with different characteristics. The searches were performed for the following countries and their official languages:

\begin{small}
\begin{description}
\item [Google:] Afghanistan, South Africa, Algeria, Angola, Saudi Arabia, Argentina, Australia, Austria, Brazil, Canada, Chile, Denmark, Egypt, Finland, France, Germany, Greece, Guatemala, India, Iraq, Ireland, Italy, Japan , Kenya, United Kingdom, South Korea, Malaysia, Mexico, Morocco, Nigeria, Paraguay, Peru, Portugal, Russia, Spain, United States, Sweden, Turkey, Ukraine, Uzbekistan, Venezuela and Zambia.
\item [Bing:] Saudi Arabia, Denmark, Austria, Germany, Greece, Australia, Canada, United Kingdom, United States, South Africa, Argentina, Spain, Mexico, Finland, Italy, Japan, South Korea, Brazil, Portugal, Russia, Turkey and Ukraine.
\end{description}
\end{small}

\subsection{Analysis}
\label{sec:analysis}

\camila{Alguma sugestão para o nome dessa seção? Não consegui pensar em nada diferente apesar de não ter gostado de 'Analysis'.}

Our main purpose is to identify whether there is a stereotype in the perception of physical attractiveness. For sake of our analysis, we distinguish two characteristics extracted from the pictures: race and age. As discussed, stereotype is a subjective concept and quantifying it through objective criteria is a challenge. In our case, we employed a {\em contrast}-based strategy. Considering race as a criteria, we check the difference between the proportions of each race for opposite queries, that is, beautiful woman and ugly woman. We consider that there is a negative stereotype of beauty in relation to a race, when the frequency of this particular race is larger when we search for ugly women compared to when we search for beautiful woman. Likewise, the stereotype is considered to be positive when the proportion is higher when we search for beautiful woman. Similarly, we say that there is a age stereotype when the ages of the women are lower in the searches for beautiful women. We characterize the occurrence of these stereotypes through seven questions:

\begin{small}
\begin{description}
\item [Q1:] Is the fraction of black women is higher when we search for ugly women than when we search for beautiful women?
\item [Q2:] Is the fraction of Asian women is higher when we search for ugly women than when we search for beautiful women?
\item [Q3:] Is the fraction of white women is higher when we search for ugly women than when we search for beautiful women?
\item [Q4:] Is the fraction of black women is lower when we search for ugly women than when we search for beautiful women?
\item [Q5:] Is the fraction of Asian women is lower when we search for ugly women than when we search for beautiful women?
\item [Q6:] Is the fraction of white women is lower when we search for ugly women than when we search for beautiful women?
\item [Q7:] Is the women's ages when we search for beautiful women are smaller than the ages of the women when we search for ugly women?
\end{description}
\end{small}

Each of these questions is associated with a test hypothesis. For the questions \textbf{Q1}, \textbf{Q2} and \textbf{Q3}, the hypothesis is:

\begin{small}
\begin{description}
\item [$H_{0}$(null hypothesis)]: The fraction of women of the specific race (i.e., black, white, Asian) is smaller when we search for ugly women, than when we search for beautiful women.
\item  [$H_{a}$(alternative hypothesis)]: The fraction of women of the specific race (i.e., black, white, Asian) is higher when we search for ugly women than when we search for beautiful women.
\end{description}
\end{small}

For the questions \textbf{Q4}, \textbf{Q5} and \textbf{Q6}:

\begin{small}
\begin{description}
\item [$H_{0}$]: The fraction of women of the specific race (black, white, Asian) is greater when we search for ugly women, if compared to the proportion of women of the race (black, white, Asian) when we search for beautiful women.
\item  [$H_{a}$]: The fraction of women of the specific race (black, white, Asian) is lower when we search for ugly women, if compared to the proportion of women of the race (black, white, Asian) when we search for beautiful women.
\end{description}
\end{small}

For the question \textbf{Q7}:

\begin{small}
\begin{description}
\item [$H_{0}$]: The age range of the beautiful women is greater than the age range of the ugly women.
\item  [$H_{a}$]: The age range of the beautiful women is lower than the age range of the ugly women.
\end{description}
\end{small}

\meira{How about the Z-score?}

\subsection{Clustering}
\label{sec:cluster}

After identifying the existence of stereotypes in the perception of physical attractiveness, we would like to discover whether there is a cohesion among these beauty stereotypes considering all data. For this we will use a clustering algorithm to identify the countries that have the same racial stereotype of beauty. Each country is represented as a point in the three-dimensional space where the dimensions are Asian, black and white z-scores.

There are several strategies for clustering, however a hierarchical clustering strategy was used in this paper because it outputs a hierarchy that can be very useful for our analysis. We used the Ward's minimum variance method \footnote{R library: https://stat.ethz.ch/R-manual/R-devel/library/stats/html/hclust.html} which is briefly described next. Using a set of dissimilarities for the objects being clustered, initially, each object is assigned to its own cluster and then the algorithm proceeds interactively. At each stage it joins the two most similar clusters, continuing until there is just a single cluster. The method aims at finding compact and spherical clusters\cite{murtagh2014ward}. Another advantage of employing a hierarchical clustering strategy is that it is not necessary to set in advance parameters such as the number of clusters of minimal similarity thresholds, allowing us to investigate various clusters configurations easily.





==> results.tex <==
\section{Results}
\label{sec:case}
\subsection{Racial Stereotype}

As presented in section~\ref{sec:method}, to verify that stereotypes exist, we will use the 7 questions ({\bf Q1}, {\bf Q2}, {\bf Q3}, {\bf Q4}, {\bf Q5}, {\bf Q6} and {\bf Q7}) and the hypothesis associated with each one of them. We assume that there is a negative stereotype of beauty in relation to a race, when the distribution of this particular race is significantly greater when we search for ugly women compared to when we search for beautiful woman and a positive one when the proportion is significantly lower.

In order to verify the significance of each of these differences we will employ the two-proportion z-test with a significance level of $0.05$. The test determines whether the hypothesized difference between the proportions differs significantly. For the first three questions, ({\bf Q1}, {\bf Q2} and {\bf Q3}), with confidence of 95\% we reject the null hypothesis when the z-score is lower than $-0.8289$ and we accept the alternative hypothesis, which is the hypothesis in study. For the questions ({\bf Q4}, {\bf Q5} and {\bf Q6}), under the same conditions, we reject the null hypothesis when the z-score is greater than $0.8289$. Detailed results of the tests are in the appendix~\ref{app2} .

\subsection{Age Stereotype}

In the second case we are working with the age distribution. Therefore, to verify our hypothesis we employ the unpaired Wilcoxon test~\ref{wilcoxon}. The null hypothesis is rejected when p-value is less than 0.05. and with 95\% of confidence we can answer YES to question {\bf Q7} (see appendix~\ref{app3} for detailed results). 

Table \ref{summary} summarizes the test results with the proportion of countries that we answer YES to each of the 7 questions (reject the null hypothesis). We can see that the results of the two search engines agree. There is a beauty stereotype in the perception of physical attractiveness, we can say that significantly the proportion of black and Asian women is greater when we search for ugly women compared to the proportion of those races when we search for beautiful women (negative stereotype). The opposite occurs with white women (positive stereotype).

\begin{table}[!h]
\centering
\begin{small}
\begin{tabular}{lcc}
\cline{2-3}
                    & \multicolumn{2}{c}{\textbf{Results}}                                   \\ \cline{2-3} 
                    & \multicolumn{1}{c|}{\textit{\textbf{Google}}} & \textit{\textbf{Bing}} \\ \cline{2-3} 
\textit{Q1 (Black)} & \multicolumn{1}{c|}{\textbf{85.71\%}}         & \textbf{76.47\%}       \\ \hline
\textit{Q2 (Asian)} & \multicolumn{1}{c|}{\textbf{26.19\%}}         & \textbf{29.41\%}       \\ \hline
\textit{Q3 (White)} & \multicolumn{1}{c|}{4.76\%}                   & 5.88\%                 \\ \hline
\textit{Q4 (Black)} & \multicolumn{1}{c|}{2.38\%}                   & 0.00\%                 \\ \hline
\textit{Q5 (Asian)} & \multicolumn{1}{c|}{4.76\%}                   & 11.76\%                \\ \hline
\textit{Q6 (White)} & \multicolumn{1}{c|}{\textbf{78.57\%}}         & \textbf{82.35\%}       \\ \hline
\textit{Q7 (Age)}   & \multicolumn{1}{c|}{\textbf{69.05\%}}         & \textbf{82.35\%}      
\end{tabular}
\caption{Summary of results for questions {\bf Q1}, {\bf Q2}, {\bf Q3}, {\bf Q3}, {\bf Q4}, {\bf Q5}, {\bf Q6} e {\bf Q7}}
\label{summary}
\end{small}
\end{table}

\subsection{Clustering}

%After identifying the existence of stereotypes in the perception of physical attractiveness, we would like to discover if there is a Global cohesion among these beauty stereotypes.

The clusters we are looking for should be cohesive and also semantically meaningful. Cohesion is achieved by the Ward's minimum variance method, but the semantic of the clusters should take into account cultural, political and historical aspects. For the results presented here we traversed the dendrogram starting from the smallest variance to the maximum variance \meira{should explain what is the variable whose variance we are talking about}, which is the root of the dendrogram. For each group of entities, we verify what they do have in common so that we may understand why they behaved similarly or not. In some cases we were not able to infer the factor that explain portions of the dendrogram and leave such investigation for future work. \meira{mandar para o future work} For now, we want to highlight positive evidence that our approach is able to identify relevant and significant stereotypes across several entities (e.g., countries).

Figure~\ref{clusters} presents the dendrograms for both search engines, we use a cutoff of 6 clusters to illustrate the process of clustering from the dendrogram structure. The centroids of the clusters are shown in Table~\ref{tabCentroids}. It is important to emphasize that when analyzing the centroids of each cluster the dimensions represent the z-score for each race. In our previous analysis we have shown that for black and Asian women, a more negative score represents a stronger negative stereotype regarding the two races. For white women, a more positive score represents a stronger positive stereotype.

\begin{figure}[!h]
  \begin{subfigure}[b]{0.6\textwidth}
          \centering
        \includegraphics[scale=0.5]{fig/dendGoogle.png}
   	\caption{Dendrogram with the cutoff of 6 clusters for Google.}  
		\label{clusteringGoogle}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.55\textwidth}
          \centering
        \includegraphics[scale=0.45]{fig/dendBing.png}
   	\caption{Dendrogram with the cutoff of 6 clusters for Bing.}   
		\label{clusteringBing}
  \end{subfigure}
  \caption{Clusters} 
  \label{clusters}
\end{figure}

In Google dendrogram, we can highlight the cluster 1 - Spain, Guatemala, Argentina, USA, Peru, Mexico, Venezuela, Chile, Brazil and Paraguay - which has a geographical semantic meaning: countries from the American continent and Spain, that just as the most of these countries has Latin origin. The centroid of this cluster (black: -3.28, Asian: 0.60, white: 2:02) indicates that for this group of countries there is a very negative stereotype regarding black women and a positive stereotype for white women. In the Cluster 2 - Ireland, Austria, Germany and Greece - we have European countries and a different stereotype (black: -1.23, Asian: -1.72, white: 2.23) since Asians have a more negative stereotype than blacks. For Cluster 4 - Russia, India, Denmark, Ukraine, South Korea, Kenya, Finland, Japan, Uzbekistan and Afghanistan - we could not identify a semantic meaning of cohesion within the group. However, the cluster has an interesting beauty stereotype (black:-0.60, Asian:0.05, white:0.28) in which the stereotype, positive or negative, regarding the races do not exist or are small. There is a coherence between the proportions of the races for the two queries, that is, for most of these countries there is no significant difference between the proportions of the races when we search for beautiful women or ugly women.

In the clustering process of Bing data, Cluster 3 (black:-1.33, Asian:2.70, white:-2.37), composed only by Japan, has the same stereotype of beauty that Cluster 5 of Google (black:-2.24, Asian:2.86, white:-1.84), composed only by Malaysia. Both are composed of just a Asian country and therefore have a very positive stereotype regarding Asian and negative stereotype  regarding black women and white women.

\begin{table}[!h]
\centering
\caption{Clusters centroids}
\label{tabCentroids}
\begin{scriptsize}
\begin{tabular}{lcccccc}
\cline{2-7}
                                         & \multicolumn{6}{c}{\textbf{Google}}                                                                                                                                                                             \\ \cline{2-7} 
\multicolumn{1}{l|}{}                    & \multicolumn{2}{c|}{\textit{\textbf{Black}}}                        & \multicolumn{2}{c|}{\textit{\textbf{Asian}}}                        & \multicolumn{2}{c|}{\textit{\textbf{White}}}                        \\ \cline{2-7} 
\multicolumn{1}{l|}{}                    & \textit{Mean}                 & \multicolumn{1}{c|}{\textit{STDEV}} & \textit{Mean}                 & \multicolumn{1}{c|}{\textit{STDEV}} & \textit{Mean}                 & \multicolumn{1}{c|}{\textit{STDEV}} \\ \hline
\multicolumn{1}{|l|}{\textit{Cluster 0}} & -2.85                         & \multicolumn{1}{c|}{0.16}           & -0.41                         & \multicolumn{1}{c|}{0.38}           & 2.65                          & \multicolumn{1}{c|}{0.12}           \\
\multicolumn{1}{|l|}{\textit{Cluster 1}} & -3.28                         & \multicolumn{1}{c|}{0.21}           & 0.60                          & \multicolumn{1}{c|}{0.31}           & 2.02                          & \multicolumn{1}{c|}{0.34}           \\
\multicolumn{1}{|l|}{\textit{Cluster 2}} & -1.23                         & \multicolumn{1}{c|}{0.22}           & -1.72                         & \multicolumn{1}{c|}{0.92}           & 2.23                          & \multicolumn{1}{c|}{0.71}           \\
\multicolumn{1}{|l|}{\textit{Cluster 3}} & -2.68                         & \multicolumn{1}{c|}{0.24}           & -1.87                         & \multicolumn{1}{c|}{0.38}           & 3.40                          & \multicolumn{1}{c|}{0.19}           \\
\multicolumn{1}{|l|}{\textit{Cluster 4}} & -0.60                         & \multicolumn{1}{c|}{0.28}           & 0.05                          & \multicolumn{1}{c|}{0.44}           & 0.28                          & \multicolumn{1}{c|}{0.73}           \\
\multicolumn{1}{|l|}{\textit{Cluster 5}} & -2.24                         & \multicolumn{1}{c|}{0.00}           & 2.86                          & \multicolumn{1}{c|}{0.00}           & -1.84                         & \multicolumn{1}{c|}{0.00}           \\ \hline
                                         & \multicolumn{1}{l}{\textbf{}} & \multicolumn{1}{l}{\textbf{}}       & \multicolumn{1}{l}{\textbf{}} & \multicolumn{1}{l}{\textbf{}}       & \multicolumn{1}{l}{\textbf{}} & \multicolumn{1}{l}{\textbf{}}       \\ \cline{2-7} 
                                         & \multicolumn{6}{c}{\textbf{Bing}}                                                                                                                                                                               \\ \cline{2-7} 
\multicolumn{1}{l|}{}                    & \multicolumn{2}{c|}{\textit{\textbf{Black}}}                        & \multicolumn{2}{c|}{\textit{\textbf{Asian}}}                        & \multicolumn{2}{c|}{\textit{\textbf{White}}}                        \\ \cline{2-7} 
\multicolumn{1}{l|}{}                    & \textit{Mean}                 & \multicolumn{1}{c|}{\textit{STDEV}} & \textit{Mean}                 & \multicolumn{1}{c|}{\textit{STDEV}} & \textit{Mean}                 & \multicolumn{1}{c|}{\textit{STDEV}} \\ \hline
\multicolumn{1}{|l|}{Cluster 0}          & -0.53                         & \multicolumn{1}{c|}{0.31}           & -0.66                         & \multicolumn{1}{c|}{0.10}           & 0.90                          & \multicolumn{1}{c|}{0.09}           \\
\multicolumn{1}{|l|}{Cluster 1}          & -1.60                         & \multicolumn{1}{c|}{0.03}           & -0.83                         & \multicolumn{1}{c|}{0.21}           & 1.75                          & \multicolumn{1}{c|}{0.15}           \\
\multicolumn{1}{|l|}{Cluster 2}          & -1.82                         & \multicolumn{1}{c|}{0.02}           & 0.47                          & \multicolumn{1}{c|}{0.74}           & 0.78                          & \multicolumn{1}{c|}{0.44}           \\
\multicolumn{1}{|l|}{Cluster 3}          & -1.33                         & \multicolumn{1}{c|}{0.00}           & 2.70                          & \multicolumn{1}{c|}{0.00}           & -2.37                         & \multicolumn{1}{c|}{0.00}           \\
\multicolumn{1}{|l|}{Cluster 4}          & -2.85                         & \multicolumn{1}{c|}{0.65}           & 0.00                          & \multicolumn{1}{c|}{0.42}           & 2.27                          & \multicolumn{1}{c|}{0.19}           \\
\multicolumn{1}{|l|}{Cluster 5}          & -2.85                         & \multicolumn{1}{c|}{0.22}           & -1.23                         & \multicolumn{1}{c|}{0.05}           & 3.20                          & \multicolumn{1}{c|}{0.23}           \\ \hline
\end{tabular}
\end{scriptsize}
\end{table}

%Cluster validation (Figure~\ref{sil}).

%\begin{figure}[!h]
%	\centering
%  \begin{subfigure}[b]{0.55\textwidth}
%          \centering
%        \includegraphics[scale=0.5]{fig/silGoogle.png}
%   	\caption{Silhouette analysis Google.}   
%		\label{silGoogle}
%  \end{subfigure}
%  \newline
%	\begin{subfigure}[b]{0.55\textwidth}
%          \centering
%        \includegraphics[scale=0.4]{fig/silBing.png}
%   	\caption{Silhouette analysis Bing.}   
%		\label{silBing}
%  \end{subfigure}
%  \caption{Silhouette analysis} 
%  \label{sil}
%\end{figure}





